Faster Algorithms for Algebraic Path Properties in RSMs with Constant Treewidth

Interprocedural analysis is at the heart of numerous applications in programming languages, such as alias analysis, constant propagation, etc. Recursive state machines (RSMs) are standard models for interprocedural analysis. We consider a general framework with RSMs where the transitions are labeled from a semiring, and path properties are algebraic with semiring operations. RSMs with algebraic path properties can model interprocedural dataflow analysis problems, the shortest path problem, the most probable path problem, etc. The traditional algorithms for interprocedural analysis focus on path properties where the starting point is \emph{fixed} as the entry point of a specific method. In this work, we consider possible multiple queries as required in many applications such as in alias analysis. The study of multiple queries allows us to bring in a very important algorithmic distinction between the resource usage of the \emph{one-time} preprocessing vs for \emph{each individual} query. The second aspect that we consider is that the control flow graphs for most programs have constant treewidth. Our main contributions are simple and implementable algorithms that support multiple queries for algebraic path properties for RSMs that have constant treewidth. Our theoretical results show that our algorithms have small additional one-time preprocessing, but can answer subsequent queries significantly faster as compared to the current best-known solutions for several important problems, such as interprocedural reachability and shortest path. We provide a prototype implementation for interprocedural reachability and intraprocedural shortest path that gives a significant speed-up on several benchmarks.

==> balanced.tex <==
\section{Balanced tree decomposition}\label{sec:balanced}

\begin{lemma}\label{lem:tree_paths}
Consider a weighted graph $G=(V,E)$ and a tree-decomposition $\Tree(G)$.
Let $u,v\in V$, and $P':\Bag_{1}, \Bag_{2},\dots,\Bag_{j}$ be the unique path in $T$ such that $u\in \Bag_{1}$ and $v\in \Bag_{j}$. For each $i\in \{1,\dots, j-1\}$ and for each path $P:u\rightsquigarrow v$, there exists a node $x_{i}\in (\Bag_{{i}}\cap \Bag_{{i+1}}\cap P)$.
\end{lemma}
\begin{proof}
Fix a number $i\in \{1,\dots, j-1\}$. We argue that for each path $P:u\rightsquigarrow v$, there exists a node $x_{i}\in (\Bag_{{i}}\cap \Bag_{{i+1}}\cap P)$.
We construct a tree $\Tree'(G)$, which is similar to $\Tree(G)$ except that instead of having an edge between bag $\Bag_{{i}}$ and bag $\Bag_{{i+1}}$, there is a new bag $\Bag$, that contains the nodes in $\Bag_{{i}}\cap \Bag_{{i+1}}$, and there is an edge between $\Bag_{{i}}$ and $\Bag$ and one between  $\Bag$ and $\Bag_{{i+1}}$. It is easy to see that $\Tree'(G)$ forms a tree-decomposition of $G$. Let $\mathcal{C}_1$, $\mathcal{C}_2$ be the two components of $\Tree(G)$ separated be $\Bag$, and w.l.o.g. $u\in \mathcal{C}_1$ and $v\in\mathcal{C}_2$. It follows by the definition of tree-decomposition that $\Bag$ is a separator of $\bigcup_{\Bag'\in \mathcal{C}_1}$ and $\bigcup_{\Bag'\in \mathcal{C}_2}$.
Hence, each path $u\rightsquigarrow v$ must go through some node $x_i$ in $\Bag$, and by construction $x_i\in \Bag_i\cap \Bag_{i+1}$.
\end{proof}


Given the tree-decomposition $\Tree(G)=(V_T, E_T)$, we assign to each bag $\Bag\in V_T$
a rank $\Rank(\Bag)\in \Nats$ according to the recursive Algorithm~\ref{algo:rank}.
Initially, we assign $\Rank(B)=\bot$ for all $B\in V_T$. 



\smallskip
\begin{algorithm}%[H]
\small
\SetAlgoNoLine
\DontPrintSemicolon
%\setstretch{1.05}
\caption{$\Rankalgo$}\label{algo:rank}
\KwIn{A component of bags $\mathcal{C}$, a flag $f$, a rank $k\in \Nats$}
\KwOut{A rank function $\Rank:\mathcal{C}\rightarrow \Nats$}
\BlankLine
\uIf{$\mathcal{C}=\{\Bag\}$ for some $\Bag$}{
Assign $\Rank(\Bag)\leftarrow k$\\
}
Perform a $\DFS$ in $\mathcal{C}$ and\\
\eIf{$f=\True$}
{Find a separator $\Bag$ that splits $\mathcal{C}$
into $\mathcal{C}_1$, $\mathcal{C}_2$, with $|\mathcal{C}_1|, |\mathcal{C}_2|\leq \frac{2\cdot |\mathcal{C}|}{3}$\\
Assign $\Rank(\Bag)\leftarrow k$\\
Recursively call $\Rankalgo$ on $\mathcal{C}_1$ with flag $\neg f$ and rank $k+1$
Recursively call $\Rankalgo$ on $\mathcal{C}_2$ with flag $\neg f$ and rank $k+1$\\
}
{
Find the first bag separator $\Bag$ that splits $\mathcal{C}$
into $\mathcal{C}_1$, $\mathcal{C}_2$, such that $\Bag$ has 
successors $\Bag_1$, $\Bag_2$ with $\Rank(\Bag_1),\Rank(\Bag_2)< k$\\
\eIf{such bag $\Bag$ exists}
{
Assign $\Rank(\Bag)\leftarrow k$\\
Recursively call $\Rankalgo$ on $\mathcal{C}_1$ with flag $\neg f$ and rank $k+1$
Recursively call $\Rankalgo$ on $\mathcal{C}_2$ with flag $\neg f$ and rank $k+1$\\
}
{
Recursively call $\Rankalgo$ on $\mathcal{C}$ with flag $\neg f$ and rank $k$\\
}
}
\end{algorithm}

Algorithm $\Rankalgo$ induces a tertiary $\emph{rank tree}$ $\Ranktree$ of $G$ such that
the root is the unique bag $\Bag$ with $\Rank(\Bag)=0$, and a bag $\Bag'$ is 
the left (right) child of a bag $\Bag$ iff $\Bag'$ is the separator of 
the sub-component $\mathcal{C}_1$ ($\mathcal{C}_2$) of the component $\mathcal{C}$
on which $\Bag$ is a separator. Level $i$ of $\Hierarchy$ contains all bags $\Bag$ with
$\Rank(\Bag)=i$.

Given the rank function $\Rank$ computed by Algorithm~\ref{algo:rank},
denote with
\begin{align*}
\Nhood(\Bag) &= \{\Bag'\in V_T:\Rank(\Bag')\leq \Rank(\Bag) \\
&\text{ and for all }\Bag''\in \Bag\rightsquigarrow \Bag',~\Rank(\Bag')\leq\Rank(\Bag'')\}\\
\end{align*}
and let $\Nhoodnodes(\Bag)=\bigcup_{\Bag'\in \Nhood(\Bag)}\Bag'$.


\begin{lemma}\label{lem:rank_assertions}
The following assertions hold:
\begin{compactenum}
\item \label{item:node}  $\forall u\in V$, $\forall \Bag_1,\Bag_2\in V_T$, if $u$ appears in bags $\Bag_1$,
$\Bag_2$ in $\Hierarchy$, then $u$ appears in their LCA $\Bag$.
\item \label{item:sep} $\forall \Bag_1,\Bag_2\in V_T$, with $\Bag_1\neq \Bag_2$ and $\Rank(\Bag_1)=\Rank(\Bag_2)=k$, 
there exists $\Bag\in \Bag_1\rightsquigarrow \Bag_2$ such that $\Rank(\Bag)<k$.
%\item \label{item:nhoodcontains}For every bag $\Bag$ and nodes $u,v\in \Nhoodnodes(\Bag)$ with $\Rank(u)\geq \Rank(v)$, we have
%$v\in \Nhoodnodes(\Bag_u)$.
\item \label{item:rank}$\max_{\Bag\in V_T} \Rank(\Bag)=O(\log n)$,
\item \label{item:nhood}$\forall \Bag\in V_T$, we have $|\Nhood(\Bag)|\leq 4$.
\end{compactenum}
\end{lemma}
\begin{proof}
We prove each item separately.
\begin{compactenum}
\item By construction, $\Bag$ is a separator of bags $\Bag_1$, $\Bag_2$ in $\Tree(G)$.
By the definition of tree-decomposition, for all $\Bag'$ in the $\Bag_1\rightsquigarrow\Bag_2$
path in $\Tree(G)$, we have $u\in \Bag'$, hence $u\in \Bag$.
\item Let $\mathcal{C}$ be the first component processed by $\Rankalgo$
that contains both $\Bag_1, \Bag_2$, for some rank $k'$. It follows that $k'<k$.
Then $\Rankalgo$ picks a separator $\Bag\neq \Bag_1,\Bag_2$ and sets 
$\Rank(\Bag)=k'$, and by the 
choice of $\mathcal{C}$, we have $\Bag\in \Bag_1\rightsquigarrow \Bag_2$.
%\item The claim follows directly from the definition of $\Nhoodnodes(\Bag)$.
\item It is clear that $\max_{\Bag\in V_T}\Rank(\Bag)$ is upper bounded by the
recursion depth of $\Rankalgo$. Because of the alternating flag, at recursion level
$i$, for each component $\mathcal{C}$ processed by $\Rankalgo$ in that level
we have $|\mathcal{C}|\leq \left(\frac{2}{3}\right)^{\lceil i/2\rceil}$. Initially
$|\mathcal{C}|=n$, and the recursion stops when $|\mathcal{C}|=1$, hence $\max_{\Bag\in V_T} \Rank(\Bag)=O(\log n)$.
\item Let $\Bag$ be a bag assigned rank when processing 
some component $\mathcal{C}$ with flag $f$,
and let $\mathcal{C}_1$, $\mathcal{C}_2$ be the two sub-components of $\mathcal{C}$ separated by $\Bag$. 
Let $\Bag'$ be a bag that is assigned a rank when $\Rankalgo$ runs on $\mathcal{C}_1$.
Similar reasoning holds when $\Bag'\in \mathcal{C}_2$.
We consider two cases. If $f=\True$,
because of \cref{item:sep} and the fact that rankings monotonically increase with recursion levels,
we have that $\Nhood(\Bag')\subseteq \Nhood(\Bag)\cup\{\Bag'\}$, and thus $|\Nhood(\Bag')|\leq |\Nhood(\Bag)|+1$.
If $f=\False$, then there exist $\Bag_1,\Bag_2\in \Nhood(\Bag)$ with $\Rank(\Bag_1),\Rank(\Bag_2)<\Rank(\Bag)$,
and either $\Bag_1,\Bag_2\in\mathcal{C}_1$ or and either $\Bag_1,\Bag_2\in\mathcal{C}_2$.
In the former case, $\Bag\in \Bag_1\rightsquigarrow \Bag_2$, hence $\Nhood(\Bag')=3$.
In the latter case, $\Nhood(\Bag')=\Nhood(\Bag)\cup\{\Bag'\}\setminus\{\Bag_1, \Bag_2\}$.
Hence, $|\Nhood(\Bag')|\leq \max(|\Nhood(\Bag)|-1, 3)$. See \cref{fig:rank_assertions} for 
an illustration of the above cases.
In the first recursion level, we have $|\Nhood(\Bag)|=1$. 
Because of the alternating flag, an easy induction on the recursion levels of $\Rankalgo$ 
concludes that for all $\Bag\in V_T$, we have $|\Nhood(\Bag)|\leq 4$, as desired.
\end{compactenum}
\end{proof}

\begin{figure}
\centering
\begin{tikzpicture}[thick,
pre/.style={<-,shorten >= 1pt, shorten <=1pt, thick},
post/.style={->,shorten >= 1pt, shorten <=1pt,  thick},
und/.style={very thick, draw=gray},
bag/.style={ellipse, minimum height=7mm,minimum width=14mm,draw=gray!80, line width=1pt},
rootbag/.style={ellipse, minimum height=7mm,minimum width=14mm,draw=black!80, line width=2.5pt},
node/.style={circle,draw=black!80, inner sep=1, minimum size=20pt, line width=1.8},
virt/.style={circle,draw=black!50,fill=black!20, opacity=0}]
\node	[node]		(x1)		at	(-2.5,-1.5)		{$1$};
\end{tikzpicture}
\caption{ }\label{fig:rank_assertions}
\end{figure}


\begin{lemma}\label{lem:rank_complexity}
Algorithm $\Rankalgo$ runs in $O(n\log n)$ time and space.
\end{lemma}
\begin{proof}
The time spent in each component $\mathcal{C}$ is $O(|\mathcal{C}|)$.
The argument in \cref{lem:rank_assertions} shows that $\Rankalgo$ will run for
$O(\log n)$ levels of recursion. For all components $\mathcal{C}$ in a fixed level,
we have $\sum_{\mathcal{C}}|\mathcal{C}|\leq n$, hence $\Rankalgo$ runs in
$O(n\log n)$ total time. The space bound follows.
\end{proof}


For every node $u\in V$, we denote with $\Bag_u$ the bag with the lowest rank
that contains $u$, i.e., $\Bag_u=\arg\min_{\Bag\in V_T:~u\in \Bag}\Rank\left(\Bag\right)$, 
and denote with $\Rank(u)=\Rank(\Bag_u)$. It is straightforward that $\Bag_u$ is
well defined for each $u\in V$, by \cref{item:node} of \cref{lem:rank_assertions}.
We say that a pair of bags $(\Bag_1$, $\Bag_2)$ \emph{form a gap} on some node $u$
if $u\in \Bag_1\cap \Bag_2$, $\Bag_1$ is an ancestor of $\Bag_2$ in $\Hierarchy$,
and for the unique path $P:\Bag_1\rightsquigarrow \Bag_2$
in $\Hierarchy$ we have that $|P|\geq 2$ and for all intermediate bags $\Bag$ in $P$ we have $x\not\in \Bag$.

\begin{lemma}\label{lem:nhood}
For every node $u$, and pair of bags $(\Bag_1$, $\Bag_2)$ that form a gap on $u$,
for every intermediate bag $\Bag$ in $P:\Bag_1\rightsquigarrow \Bag_2$, 
we have that $\Bag_1\in \Nhood(\Bag)$.
\end{lemma}
\begin{proof}
Fix arbitrarily such a $\Bag$, and it follows that $\Rank(\Bag_2)>\Rank(\Bag)$.
Let $P_1:\Bag_2\rightsquigarrow \Bag_1$ and $P_2:\Bag\rightsquigarrow \Bag_2$
be paths in $\Tree(G)$. We argue that for all intermediate bags $\Bag'$ in $P_1$ and $P_2$, we have
that $\Rank(\Bag')>\Rank(\Bag)$. 

First, examine the case that $\Bag'$ is an intermediate bag in $P_1$
(the statement holds trivially if no such $\Bag'$ exists). We argue that $\Bag'$ is
a descendant of $\Bag_2$ in $\Hierarchy$. Indeed, $\Bag'$ cannot be
an ancestor of $\Bag_1$, since then $\Bag_1$ and $\Bag_2$ would be 
separated by $\Bag'$ in $\Hierarchy$, and $\Bag_1$ would not be
an ancestor of $\Bag_2$. Hence $\Bag'$ is a descendant of $\Bag_1$ in
$\Hierarchy$, and by \cref{item:node} of \cref{lem:rank_assertions},
$u$ appears in the LCA of $\Bag'$, $\Bag_2$. Since $P$
forms a gap on $u$, the LCA must be $\Bag_2$.

Second, examine the case that $\Bag'$ is an intermediate bag in $P_2$.
If $\Rank(\Bag')\leq \Rank(\Bag)$, then $\Bag$ and $\Bag_2$ would $\Bag'$
be the left and right child of $\Bag'$ in $\Hierarchy$, hence $\Bag$ would not be
an ancestor of $\Bag_2$.

Hence, we have shown that all intermediate nodes $\Bag'$ in the path $P_3:\Bag\rightsquigarrow \Bag_1$ in
$\Tree(G)$ have rank $\Rank(\Bag')> \Rank(\Bag)$, thus $\Bag_1\in \Nhood(\Bag)$, as desired.
\end{proof}



\smallskip
\begin{algorithm}%[H]
\small
\SetAlgoNoLine
\DontPrintSemicolon
%\setstretch{1.05}
\caption{$\Balancealgo$}\label{algo:balancealgo}
\KwIn{A hierarchy $\Hierarchy$}
\KwOut{A balanced tree-decomposition $\Tree'(G)$ of $G$}
\BlankLine
\ForEach{$\Bag\in V_T$}{
Set $\Bag\leftarrow \Bag\cup \bigcup_{\Bag'\in \Nhood(\Bag)}\Bag'$
}
\Return{$\Hierarchy$}
\end{algorithm}


\begin{lemma}\label{lem:balance_correctness}
$\Tree'(G)$ is a balanced tree-decomposition of $G$.
\end{lemma}
\begin{proof}
The height of $\Tree'(G)$ is the same as the height of $\Hierarchy$, hence it is $O(\log n)$.
We argue that $\Tree'(G)$ is a tree decomposition of $G$. It is straightforward that $\Tree'(G)$
covers nodes and edges of $G$, because every bag of $\Tree(G)$ is a subset of a bag of $\Tree(G)$.
It remains to show that every node $u$ appears in a continuous sub-tree of $\Tree'(G)$.
Assume towards contradiction otherwise. Then there exists a pair of bags $(\Bag_1$, $\Bag_2)$ that forms
a gap for $u$ in $\Tree'(G)$, and thus in $\Hierarchy$. But then for every intermediate bag $\Bag$ in
the path $P:\Bag_1\rightsquigarrow \Bag_2$ we have $\Bag_1\in \Nhood(\Bag)$, and since
$u\in \Bag_1$, after $\Balancealgo$ processes $\Bag$, we have $u\in \Bag$, a contradiction.
The desired result follows.
\end{proof}
